Hallucinating IDT Descriptors and I3D Optical Flow Features for Action Recognition with CNNs

In this paper, we revive the use of old-fashioned handcrafted video representations for action recognition and put new life into these techniques via a CNN-based hallucination step. Despite of the use of RGB and optical flow frames, the I3D model (amongst others) thrives on combining its output with the Improved Dense Trajectory (IDT) and extracted with its low-level video descriptors encoded via Bag-of-Words (BoW) and Fisher Vectors (FV). Such a fusion of CNNs and handcrafted representations is time-consuming due to pre-processing, descriptor extraction, encoding and tuning parameters. Thus, we propose an end-to-end trainable network with streams which learn the IDT-based BoW/FV representations at the training stage and are simple to integrate with the I3D model. Specifically, each stream takes I3D feature maps ahead of the last 1D conv. layer and learns to `translate' these maps to BoW/FV representations. Thus, our model can hallucinate and use such synthesized BoW/FV representations at the testing stage. We show that even features of the entire I3D optical flow stream can be hallucinated thus simplifying the pipeline. Our model saves 20-55h of computations and yields state-of-the-art results on four publicly available datasets.

==> suppl3.tex <==


\begin{figure}[t]%htbp % left bottom right top
%\hspace{0.5cm}%
\centering%%%%
\vspace{-0.3cm}
%
\begin{subfigure}[b]{0.492\linewidth}
\centering\includegraphics[trim=0 0 0 0, clip=true,width=0.95\linewidth]{images_supp/exp2-1.pdf}
%\vspace{-0.2cm}
\caption{\label{fig:str21} BoW FC (train)}
%\captionof{subfigure}{aaa\label{fig:stra}}
%\vspace{0.2cm}
\end{subfigure}
%
\begin{subfigure}[b]{0.492\linewidth}
\centering\includegraphics[trim=0 0 0 0, clip=true,width=0.95\linewidth]{images_supp/exp2-2.pdf}
%\vspace{-0.2cm}
\caption{\label{fig:str22} BoW FC (test)}
%\captionof{subfigure}{bbb\label{fig:strb}}
%\vspace{0.2cm}
\end{subfigure}
%
%
%
\vspace{-0.6cm}
\caption{Evaluation of the square difference between the hallucinated and ground truth representations on HMDB-51 (split 1). We use ({\em BoW FC}) streams with sketching and PN.}
\vspace{-0.1cm}
%\captionof{figure}{sfsd}
\label{fig:mse1a}
\end{figure}


\begin{figure}[t]%htbp % left bottom right top
%\hspace{0.5cm}%
\centering%%%%
\vspace{-0.3cm}
%
%
%
\begin{subfigure}[b]{0.492\linewidth}
\centering\includegraphics[trim=0 0 0 0, clip=true,width=0.95\linewidth]{images_supp/exp2-3.pdf}
%\vspace{-0.2cm}
\caption{\label{fig:str23} FV1 FC (train)}
%\captionof{subfigure}{cccc\label{fig:strc}}
%\vspace{0.2cm}
\end{subfigure}
%
\begin{subfigure}[b]{0.492\linewidth}
\centering\includegraphics[trim=0 0 0 0, clip=true,width=0.95\linewidth]{images_supp/exp2-5.pdf}
%\vspace{-0.2cm}
\caption{\label{fig:str25} FV2 FC (train)}
%\captionof{subfigure}{ddd\label{fig:strd}}
%\vspace{0.2cm}
\end{subfigure}
%
%
%
%
%
%
\vspace{-0.6cm}
\caption{Evaluation of the square difference between the hallucinated and ground truth representations on HMDB-51 (split 1). We use ({\em FV FC}) streams with sketching and PN.}
\vspace{-0.1cm}
%\captionof{figure}{sfsd}
\label{fig:mse1b}
\end{figure}




\begin{figure}[t]%htbp % left bottom right top
%\hspace{0.5cm}%
\centering%%%%
\vspace{-0.3cm}
%
%
%
\begin{subfigure}[b]{0.492\linewidth}
\centering\includegraphics[trim=0 0 0 0, clip=true,width=0.95\linewidth]{images_supp/exp3-1.pdf}
%\vspace{-0.2cm}
\caption{\label{fig:str31} BoW Conv (train)}
%\captionof{subfigure}{aaa\label{fig:stra}}
%\vspace{0.2cm}
\end{subfigure}
%
\begin{subfigure}[b]{0.492\linewidth}
\centering\includegraphics[trim=0 0 0 0, clip=true,width=0.95\linewidth]{images_supp/exp3-2.pdf}
%\vspace{-0.2cm}
\caption{\label{fig:str32} BoW Conv (test)}
%\captionof{subfigure}{bbb\label{fig:strb}}
%\vspace{0.2cm}
\end{subfigure}
%
\comment{
\begin{subfigure}[b]{0.245\linewidth}
\centering\includegraphics[trim=0 0 0 0, clip=true,width=0.95\linewidth]{images_supp/exp3-3.pdf}
%\vspace{-0.2cm}
\caption{\label{fig:str33} FV1 Conv (train)}
%\captionof{subfigure}{cccc\label{fig:strc}}
%\vspace{0.2cm}
\end{subfigure}
%
\begin{subfigure}[b]{0.245\linewidth}
\centering\includegraphics[trim=0 0 0 0, clip=true,width=0.95\linewidth]{images_supp/exp3-5.pdf}
%\vspace{-0.2cm}
\caption{\label{fig:str35} FV2 Conv (train)}
%\captionof{subfigure}{ddd\label{fig:strd}}
%\vspace{0.2cm}
\end{subfigure}
}
%
%
\vspace{-0.6cm}
\caption{Evaluation of the square difference between the hallucinated and ground truth representations on HMDB-51 (split 1). We use ({\em Conv}) streams.}
\vspace{-0.1cm}
%\captionof{figure}{sfsd}
\label{fig:mse2}
\end{figure}



Below we asses (i) the hallucination quality, (ii) provide additional results for higher resolution frames on MPII, and (iii) we provide further details of our pre-processing not detailed in the main submission.

%%%%%%%%% BODY TEXT
\section{Hallucination Quality}
\label{sec:mse}



%\emptybox[8cm]{4.5cm}



Below, we provide an analysis of the quality of hallucination of the BoW/FV streams compared to the ground-truth BoW/FV feature vectors. Figure \ref{fig:mse} presents histograms of the square difference between the hallucinated features and ground-truth ones. Specifically, we plot histograms of $\{(\tilde{\psi}_{(bow),mn}-\psi_{(bow),mn})^2, m\!\in\!\idx{1000}, n\!\in\!\mathcal{N}\}$, where index $m$ runs over features $m\!\in\!\idx{1000}$ and $n\!\in\!\mathcal{N}$ runs over each video. Counts for training and testing splits are normalized by 1000 (the number of features) and the number of training and testing videos, respectively. The histograms are computed over bins of size $0.01$ thus allowing us to simply plot continuously looking lines instead of bins.

Figure \ref{fig:str21} shows that the BoW ground-truth descriptors for the training split are learnt closely by our BoW hallucinating unit based on FC layers ({\em FC}). We capture histograms for epochs $1,5,15,25$ in colors interpolated from red to blue. As one can see, in early epochs, the peak around the first bin is small. As the epochs progress, the peak around the first bin becomes prominent while further bins decrease in size. This indicates that as the training epochs progress, the approximation error becomes smaller and smaller.



Figure \ref{fig:str22} shows that the BoW ground-truth descriptors for the testing split are also approximated closely by the hallucinated BoW descriptors.

We compared histograms for testing and training slits for BoW, first- and second-order FV and observed small differences only. Such a comparison can be conducted by computing the ratio of testing to training bins and it reveals variations between $0.8\times$ and $1.25\times$. Thus, without the loss of clarity, we skip showing plots for FV testing splits.

Figures \ref{fig:str23} and \ref{fig:str25} show that the first- and second-order FV terms ({\em FV1}) and ({\em FV2}) can be also learnt closely by our hallucinating units. We show only the quality of approximation on the training split as behavior on testing splits matches closely the behavior on training splits.

Figures \ref{fig:str31} and \ref{fig:str32} show  the similar learning/approximation trend for BoW training and testing. %, and the first- and second-order FV terms (training only)  given our hallucinating unit based on Convolutional layers ({\em Conv}). However, it appears that ({\em Conv}) learns slower to hallucinate FV descriptors if compared to BoW descriptors. We expect that our ({\em Conv}) unit has not enough learning capacity to fully approximate these representations.


\section{Higher Resolution Frames on MPII}
\label{sec:mpii_bb}




\begin{table}[t]%htbp % left bottom right top
\parbox{.99\linewidth}{
\setlength{\tabcolsep}{0.12em}
\renewcommand{\arraystretch}{0.70}
%\fontsize{9}{9}\selectfont
\hspace{-0.3cm}
%\centering
\begin{tabular}{ c | c | c | c | c | c | c | c | c }
 & {\em sp1} & {\em sp2} & {\em sp3} & {\em sp4} & {\em sp5} & {\em sp6} & {\em sp7} & mAP \\
\hline
\kern-0.5em {\fontsize{8}{9}\selectfont HAF*+BoW halluc.}      		 & $78.8$ & $75.0$ & $84.1$ & $76.0$ & $77.0$ & $78.3$ & $75.2$ & $77.8\%$\\
\kern-0.5em {\fontsize{7.5}{9}\selectfont HAF*+BoW hal.+MSK/PN}   & $80.1$ & $79.2$ & $84.8$ & $83.9$ & $80.9$ & $78.5$ & $75.5$ & $80.4\%$\\
\hline
\kern-0.5em {\fontsize{8}{9}\selectfont HAF$^\bullet$+BoW halluc.}      		     & $78.8$ & $78.3$ & $84.2$ & $77.4$ & $77.1$ & $78.3$ & $75.2$ & $78.5\%$\\
\kern-0.5em {\fontsize{7.5}{9}\selectfont HAF$^\bullet$+BoW hal.+MSK/PN}   & $80.8$ & $80.9$ & $85.0$ & $83.9$ & $82.0$ & $79.8$ & $79.6$ & $\mathbf{81.7}\%$\\
\hline
\end{tabular}
\vspace{0.02cm}%\\
}
%
%
\caption{Evaluations on  MPII. The ({\em HAF*+BoW halluc.}) is our pipeline with the BoW stream, ({\em *}) denotes human-centric pre-processing for 256 pixels (height) while ({\em HAF*+BoW hal.+MSK/PN}) denotes our pipeline with multiple sketches per BoW followed by Power Norm ({\em PN}). By analogy, ({\em$^\bullet$}) denotes human-centric pre-processing for 512 pixels (height).}
\vspace{-0.2cm}
\label{tab:mpiif2}
\end{table}


For human-centric pre-processing on MPII denoted by ({\em*}) in the main submission, we observed that the bounding boxes used for extraction of the human subject are of low resolution. Thus, we decided to firstly resize RGB frames to 512 pixels (height) rather than 256 pixels (as in our main submission) and then compute the corresponding optical flow, and perform extraction of human subjects for which the resolution thus increased $2\!\times$.

The ({\em HAF*+BoW halluc.}), our pipeline with the BoW stream, and  ({\em HAF*+BoW hal.+MSK/PN}) with multiple sketches and PN are computed for the standard 256 pixels (height) denoted by ({\em*}) are given in Table \ref{tab:mpiif2}. Note that results for ({\em*}) are taken from our main submission.

The ({\em HAF$^\bullet$+BoW halluc.}), our pipeline with the BoW stream, and  ({\em HAF$^\bullet$+BoW hal.+MSK/PN}) pipeline are analogous pipelines but computed for the increased 512 pixel resolution (height) denoted by ({\em$^\bullet$}). According to the table, increasing the resolution $2\!\times$ prior to human detection, extracting subjects in higher resolution and  scaling (to the 256 size for shorter side) yields 1.3\% improvement in accuracy.




\section{Data Pre-processing}
\label{sec:preproc}

 For HMDB-51 and YUP++, we use the data augmentation strategy described in the original authors' papers (\eg, random crop of videos, left-right flips on RGB and optical flow frames. For testing, center crop, no flipping are used.

For the MPII dataset with human-centric pre-processing, human detector is used first. Then, we crop  randomly around the bounding box of human subject (we include it). Finally, we allow scaling,  zooming in, and left-right flips. For longer videos, we sample sequences to form a 64-frame sequence. For short videos (less than 64 frames), we loop the sequence many times to fit its length to the expected input length. 
%
Lastly, we scale the pixel values of RGB and optical flow frames to the range between $-1$ and $1$.
